Pretrained Transformers for Simple Question Answering over Knowledge Graphs

Answering simple questions over knowledge graphs is a well-studied problem in question answering. Previous approaches for this task built on recurrent and convolutional neural network based architectures that use pretrained word embeddings. It was recently shown that finetuning pretrained transformer networks (e.g. BERT) can outperform previous approaches on various natural language processing tasks. In this work, we investigate how well BERT performs on SimpleQuestions and provide an evaluation of both BERT and BiLSTM-based models in datasparse scenarios.

==> entityrecalls_all.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l c c c c}
         R@N & BiLSTM & BiLSTM & BERT \\
             & \cite{buboqa} & (ours) & \\
         \midrule
1   & 67.8 & 76.45 & 77.17 & \\
5   & 82.6 & 87.46 & 88.18 & \\
20  & 88.7 & 91.47 & 92.13 & \\
50  & 91.0 & 93.07 & 93.71 & \\
150 & -- & 94.88 & 95.4 & \\
    \end{tabular}
    \caption{Entity recall on validation set.}
    \label{tab:entityrecalls:dev}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{l c c c c}
         R@N & BiLSTM & BiLSTM & BERT \\
             & \cite{buboqa} & (ours) & \\
         \midrule
1   & 67.8 & 76.45 & 77.17 & \\
5   & 82.6 & 87.46 & 88.18 & \\
20  & 88.7 & 91.47 & 92.13 & \\
50  & 91.0 & 93.07 & 93.71 & \\
150 & -- & 94.88 & 95.4 & \\
    \end{tabular}
    \caption{Entity recall on test set.}
    \label{tab:entityrecalls:test}
\end{table}


# Raw results for dev (100%): 
0.2219 % corrected (end before start)
95.65 % accuracy after postprocessing
98.86 % overlap after postprocessing
77.17 % R@1
88.18 % R@5
92.13 % R@20
93.71 % R@50
95.4 % R@150

# raw results for test (100%)
0.1199 % corrected (end before start)
95.35 % accuracy after postprocessing
98.97 % overlap after postprocessing
75.6 % R@1
87.44 % R@5
91.59 % R@20
93.2 % R@50
95.07 % R@150

==> entityrecalltable.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l c c c c}
         R@N & BiLSTM & BiLSTM & BERT \\
             & \cite{buboqa} & (ours) & \\
         \midrule
1   & 67.8 & 76.45 & 77.17 & \\
5   & 82.6 & 87.46 & 88.18 & \\
20  & 88.7 & 91.47 & 92.13 & \\
50  & 91.0 & 93.07 & 93.71 & \\
150 & -- & 94.88 & 95.4 & \\
    \end{tabular}
    \caption{Entity recall on validation set.}
    \label{tab:entityrecalls:dev}
\end{table}


==> othertables.tex <==

\begin{table*}[]
    \centering
    \begin{tabular}{l c c c c c c c}
                           & 2.5\% & 5\%         & 10\%         & 25\%          & 50\%          & 75\%         & 100\% \\
                           & (1k9)   & (3k8)      & (7k6)       & (18k9)       & (37k9)       & (56k8)      & (75k7) \\
    \midrule
%BiLSTM+BERT Emb            & 25.3        & 57.1        & 67.1       & 74.9        & 81.3         & 87.0          & 89.3          & 91.0         & 92.0 \\
BiLSTM                     & 26.5  & 41.0        & 56.3         & 72.4          & 79.0          & 81.3         & 82.8\\
BERT                       & 29.6*  & 48.6        & 67.5         & 76.5          & 80.1          & 82.6         & 83.6\\
    \end{tabular}
    \caption{Best observed relation prediction accuracies as a function of fraction of data retained. Evaluated on validation set. (*) indicates a cosine learning rate schedule with restarts --- in extremely low data scenarios for relation classification, this seems to yield better results than the cosine learning rate decay used everywhere else.}
    \label{tab:relacc:frac}
\end{table*}


\begin{table}[]
    \centering
    \begin{tabular}{l c c c}
         &  Accuracy & Avg. F1 & F1* \\
         \midrule
BiLSTM~\cite{buboqa} & -- & -- & 93.1\\
CRF~\cite{buboqa} & -- & -- & 90.2 \\
\midrule
%BiLSTM + Emb  & 92.0 & 96.6 & 96.5 \\
BiLSTM (ours)        & 93.8 & 97.0 & 97.1 \\
BERT (ours)          & 95.6 & 97.8 & 97.9 \\
    \end{tabular}
    \caption{Entity span prediction performance, measured by span accuracy, average span F1 and dataset-wide F1 on word level (F1*). Evaluated on validation set.}
    \label{tab:spanresults}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{l c}
         &  Accuracy \\
         \midrule
BiGRU~\cite{buboqa} & 82.3 \\
CNN~\cite{buboqa} & 82.8 \\
\midrule
BiLSTM (ours) & 82.8 \\
BERT (ours) &  83.6
    \end{tabular}
    \caption{Relation prediction performance, measured by accuracy (R@1). Evaluated on validation set.}
    \label{tab:relresults}
\end{table}

